A nonlinear model predictive control framework using reference generic terminal ingredients -- extended version

In this paper, we present a quasi infinite horizon nonlinear model predictive control (MPC) scheme for tracking of generic reference trajectories. This scheme is applicable to nonlinear systems, which are locally incrementally stabilizable. For such systems, we provide a reference generic offline procedure to compute an incrementally stabilizing feedback with a continuously parameterized quadratic quasi infinite horizon terminal cost. As a result we get a nonlinear reference tracking MPC scheme with a valid terminal cost for general reachable reference trajectories without increasing the online computational complexity. As a corollary, the terminal cost can also be used to design nonlinear MPC schemes that reliably operate under online changing conditions, including unreachable reference signals. The practicality of this approach is demonstrated with a benchmark example. This paper is an extended version of the accepted paper [1], and contains additional details regarding \textit{robust} trajectory tracking (App.~B), continuous-time dynamics (App.~C), output tracking stage costs (App.~D) and the connection to incremental system properties (App.~A).

==> Increm_Stab_0.tex <==
%!TEX root = ./Tracking_Journal.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{(Local) Incremental exponential stabilizability}
\label{sec:loc_stab_0}
In the following we clarify the connection between incremental stabilizability properties and the terminal ingredients.
\begin{definition}
\label{def:increm_stab}
A set of reference trajectories $r$ specified by some dynamic inclusion $r(t+1)\in\mathcal{R}(r(t))$ is locally incrementally exponentially stabilizable for the system~\eqref{eq:sys},  if there exist constants $\rho\in(0,1),M,c>0$ and a control law $\kappa(x,r)$, such that for any initial condition
 satisfying $\|x(0)-x_r(0)\|\leq c$, the trajectory $x(t)$ with $x(t+1)=f(x(t),\kappa(x(t),r(t)))$ satisfies $\|x(t)-x_r(t)\|\leq M\rho^t\|x(0)-x_r(0)\|$,~$\forall t\geq 0$. 
\end{definition}
This definition is closely related to the concept of universal exponential stabilizability~\cite{manchester2017control}, which characterizes the stabilizability of arbitrary trajectories in continuous-time. 
One of the core differences in the definitions is the treatment of constraints, i.e. we study stabilizability of classes of trajectories $r$ that satisfy certain constraints, compare Assumption~\ref{ass:ref} and Remark~\ref{rk:ref}. 
This difference is crucial when discussing local versus global stabilizability and constrained control. 

The following proposition shows that the conditions in Lemma~\ref{lemma:lpv} directly imply local incremental exponential stabilizability of the reference trajectory. 
\begin{proposition}
\label{prop:increm}
Suppose that there exist matrices $P_f(r),~K_f(r)$ that satisfy the conditions in Lemma~\ref{lemma:lpv}. 
Then the control law $k_f(x,r)=u_r+K_f(r)(x-x_r)$ locally incrementally exponentially stabilizes any reference $r$ satisfying Assumption~\ref{ass:ref}.
\end{proposition}
\begin{proof}
The following proof follows the arguments of~\cite[Prop.~1,2]{kohlernonlinear19}. 
For any $\|x(0)-x_r(0)\|\leq c$ with $c=\sqrt{\alpha/c_{u}}$, we have $x(0)\in\mathcal{X}_f(r)$, with $\alpha,~c_{u}$ according to Lemma~\ref{lemma:lpv}. 
Thus, the terminal cost $V_f(x,r)$ is a local incremental Lyapunov function that satisfies 
\begin{align*}
V_f(x(t+1),r(t+1))\leq \rho^2 V_f(x(t),r(t)),~ \rho^2=1-\dfrac{\lambda_{\min}(Q)}{c_u},
\end{align*}
and thus 
\begin{align*}
\|x(t)-x_r(t)\|\leq {\rho}^tM \|x_r(0)-x(0)\|,\quad M=\sqrt{{c_u}/{c_l}}.
\end{align*}
\end{proof}
\begin{remark}
\label{rk:increm}
This result establishes local incremental stabilizability with the incremental Lyapunov function $V_f(x,r)$ based on properties of the linearization, compare~\cite[Prop.~1]{kohlernonlinear19}. 
This system property is a natural extension of previous works on incremental stability and corresponding incremental Lyapunov functions, see~\cite{angeli2002lyapunov},~\cite[Ass.~1]{kohlernonlinear19}.  %tran2016incremental
This property implies stabilizability of $(A(r),~B(r))$ around any (fixed) steady-state $r^+=r$, but it does not necessarily imply stabilizability of $(A(r),~B(r))$ for arbitrary $r\in\mathcal{Z}_r$, as $P_f(r)$ might decrease along the trajectory. 

For continuous-time systems, an analogous result exists based on contraction metrics and universal stabilizability~\cite{manchester2017control}. 
\end{remark}
The following proposition shows that in the absence of constraints we recover non-local results similar to~\cite{manchester2017control}. 
\begin{proposition}
\label{prop:univ}
Consider $\mathcal{Z}_r=\mathcal{Z}=\mathbb{R}^{n+m}$. 
Suppose that there exist matices $P_f(r),~K_f(r)$ that satisfy the conditions in Lemma~\ref{lemma:lpv}. 
Assume further that $c_lI\leq P_f(r)\leq c_uI$ for all $r\in\mathbb{R}^{n+m}$ with some constants $c_l,~c_u$ and $K_f(r)=K(x_r)$. 
Then any  reference $r$ satisfying Assumption~\ref{ass:ref} is exponentially incrementally stabilizable with the control law 
\begin{align*}
\kappa(x,r)=K(x)x-K(x_r)x_r+u_r,
\end{align*} 
i.e., for any initial condition $x(0)\in\mathbb{R}^n$ the state trajectory $x(t+1)=f(x(t),\kappa(x(t),r(t)))$ satisfies $\|x(t)-x_r(t)\|\leq M\rho^t\|x(0)-x_r(0)\|$. 
\end{proposition}
\begin{proof}
Consider an auxiliary (pre-stabilized) system defined by $\tilde{f}(x,v)=f(x,K(x)x+v)$. 
Consider a reference $r$ generated by some input trajectory $u_r$ with the system dynamics~\eqref{eq:sys} (Ass.~\ref{ass:ref}) and some initial condition $x_r(0)$ resulting in the state reference $x_r$. 
Now, consider a reference $\tilde{r}$ generated by the input $v_r(t)=u_r(t)-K(x_r(t))x_r(t)$ with the system dynamics according to $\tilde{f}$ and the same initial condition. 
Due to the definition of the auxiliary system we have  $\tilde{x}_r(t)=x_r(t)$, $\forall t\geq 0$. 
For an arbitrary, but fixed input $v$, stability of the reference trajectory is equivalent to contractivity of the nonlinear time-varying system $\tilde{f}(x,t)$. 
This can be established with the contractivity metric $P_f(r(t))=P_f(x_r(t),t)$, compare~\cite{lohmiller1998contraction}. 
\end{proof}
In the absence of constraints, it is crucial that $P_f$ has a constant lower and upper bound.  
If the matrix $K_f$ depends on the full reference $r$ (not just $x_r$), the controller $\kappa$ in Proposition~\ref{prop:univ} is not necessarily well defined. 
%
\begin{remark}
\label{rk:track_vs_stab}
The relation between the controller $k_f$ (Prop.~\ref{prop:increm}) and $\kappa$ (Prop.~\ref{prop:univ}), is that of reference tracking versus pre-stabilization. 
The first one is more natural in the context of tracking MPC and contains existing results for the design of terminal ingredients as special cases~\cite{chen1998quasi,faulwasser2011model,aydiner2016periodic}. 
The second controller $\kappa$ allows for non-local stability results and is more suited for unconstrained control problems~\cite{manchester2017control}. 
For constant matrices $K$ the two controllers are equivalent, but the incremental Lyapunov functions (and thus terminal costs) are differently parameterized ($P_f(r)$, $P_f(x,u)$).  
\end{remark}
%
\begin{remark}
\label{rk:term_other}
The problem of computing reference generic terminal ingredients is equivalent to computing an incrementally stabilizing controller and is thus strongly related to the computation of robust positive invariant (RPI) tubes in nonlinear robust MPC schemes, compare~\cite{bayer2013discrete,kohler2018novel}. 
For comparison, in~\cite{yu2010robust,yu2013tube} constant matrices $P_f,~K_f$ are computed that certify incremental stability for continuous-time systems (by considering small Lipschitz nonlinearities or by describing the linearization as a convex combination of different linear systems). 
This approach can be directly extended to more general nonlinear systems using the proposed terminal ingredients. 
In particular, by changing the stage cost to 
\begin{align*}
\ell(x,u,r)=\|u-u_r+K(x_r)x_r-K(x)x\|_R^2 %\|x-x_r\|_Q^2+
\end{align*}
 one can design a nonlinear version of~\cite{chisci2001systems}, compare also~\cite{kohler2018novel}. 
A detailed description of a corresponding nonlinear robust tube based (tracking) MPC scheme based on incremental stabilizability can be found in~\cite[App.~A]{JK_QINFJournal_extended}. % and~\cite{}.% Appendix~\ref{sec:app_robust}. 
\end{remark}
%
\begin{remark}
\label{rk:non_quadratic}
In case a system is not exponentially stabilizable~\cite{muller2017quadratic}, it might be possible to make a nonlinear transformation resulting in a quadratically stabilizable system. 
%, compare numerical example in Section~\ref{sec:num}. 
% (see for example nonlinear systems in normal form~\cite{isidori2013nonlinear}). %\cite{byrnes1991asymptotic}.
\end{remark}
